Knowledge Transfer across Imaging Modalities Via Simultaneous Learning of Adaptive Autoencoders for High-Fidelity Mobile Robot Vision

Enabling mobile robots for solving challenging and diverse shape, texture, and motion related tasks with high fidelity vision requires the integration of novel multimodal imaging sensors and advanced fusion techniques. However, it is associated with high cost, power, hardware modification, and computing requirements which limit its scalability. In this paper, we propose a novel Simultaneously Learned Auto Encoder Domain Adaptation (SAEDA)-based transfer learning technique to empower noisy sensing with advanced sensor suite capabilities. In this regard, SAEDA trains both source and target auto-encoders together on a single graph to obtain the domain invariant feature space between the source and target domains on simultaneously collected data. Then, it uses the domain invariant feature space to transfer knowledge between different signal modalities. The evaluation has been done on two collected datasets (LiDAR and Radar) and one existing dataset (LiDAR, Radar and Video) which provides a significant improvement in quadruped robot-based classification (home floor and human activity recognition) and regression (surface roughness estimation) problems. We also integrate our sensor suite and SAEDA framework on two real-time systems (vacuum cleaning and Mini-Cheetah quadruped robots) for studying the feasibility and usability.

==> old_text.tex <==
%Many robotic sensing technologies such as Lidar and Radar enables mobile robot versatility and efficiency in solving complex robotic autonomy, navigation and vision problems. However, recent advancement of deep learning based domain adaptation techniques have the capability to empower noisy (say Radar) signal by transferring knowledge learned from less erroneous (say Lidar) signals. In this paper, we propose \emph{SAEDA}, an Adaptive Autoencoder with Simultaneous learning framework that combines a novel auto-encoder-based simultaneous learning technique to empower noisy sensing by transferring domain knowledge from less noisy sensor signal. \emph{SAEDA} trains both source and target auto-encoders using a carefully designed simultaneous learning scheme on a single graph with a novel objective function to obtain the domain invariant feature space between source and target domains from simultaneously collected data points. Additionally, it provides a novel classification technique utilizing learned domain invariant feature spaces from source and transferring to the target that improves the target classification both with and without source labels. We evaluate the performance of \emph{SAEDA} from real-time collected data on three use cases: (i) activity recognition, (ii) surface characterization and (iii) surface roughness estimation which provides significant improvement over the state-of-art methods. Finally, we integrate our prototype hardware and framework in MIT Mini-Cheetah, a 0.3 m tall, 9 kg quadruped robot and run a feasibility study in outdoor surveillance.

%Lidar (light detection and ranging) sensor enables mobile robot versatility and efficiency in solving complex robotic autonomy, navigation and vision problems. Lidar holds superiority to Radar in many ways such as in solving complex robotic autonomy, navigation and vision problems due to its less noisy 3D point-cloud reconstructions of objects. However, recent advancement of imaging radar technology that enables 2D/3D reconstructions of objects more accurately than ever, provides extreme promises in small robotic sensing due to its affordability, reliability, surface properties detectability and longer eyesight. Moreover, the high cost of Lidar sensor and necessity of high computation for analyzing its dense point clouds, Radar could be a promising alternative to Lidar for mobile robots to solve the problems of remote surface characterization, surface roughness estimation, human activity recognition and many more.


%\bt{DH: I think that we need to have a table or paragraph to explain Radar sensor - I think that robotics generally are not very familiar with the sensor.}

%Mobile robots are the focus of a great deal of current research in robotics due to their capability of solving many complex issues related to agriculture [], product deliveries [], healthcare [] and many others. Despite of the immense potentials, mobile robots have several fundamental limitations. For example, MIT Mini-Cheetah quadruped robot \cite{Katz2019MiniCA}, that enables dynamic locomotion capabilities in mobile robotics providing many promising applications, do not have enough space and power to integrate Lidar like efficient but power hungry sensors to accommodate best of its outcomes. Moreover, the high cost of Lidar sensor and necessity of high computation for analyzing its dense point clouds, Radar could be a promising alternative to Lidar for mobile robots to solve the problems of remote surface characterization, surface roughness estimation, human activity recognition and many more.



%% more scenario of Lidar and Radar in Small Robot Locomotion

%Recent advancement of deep domain adaptation facilitates significant improvement in target domain classification performance in presence of label scarcity \cite{tzeng2017adversarial}, noise \cite{ csurka2017domain} and heterogeneity \cite{tzeng2017adversarial} by transferring knowledge from superior source data. The key advantages of using deep domain adaptation networks is the ability to extract domain invariant features and transferring knowledge among those complex feature spaces which diminishes deficiencies of target data.



%\section{Related Works}
%\emph{SAEDA} strongly stands on the base of solving the problems induced by state-of-art domain adaptation techniques (adversarial network- and discrepancy-based) sustaining their capabilities using a simultaneous learning mechanism and its application in solving noisy Radar based mobile robotic surveillance related problems, such as human activity recognition, object characterization and surface characterization.

%\subsection{Transferring Knowledge from Lidar to Radar}
%The connection between lidar and radar is a popular topic for range sensing in recent years for mobile robotics and automated car driving. Compared to lidar based place recognition, locomotion and surface mapping system, there are few research search on radar range data.  

%\subsection{Domain Adaptation in Computer Vision}
%The sole target of all of the deep domain adaptation method is to learn a shared feature representation across different domains by minimizing the distribution discrepancies. Based on the feature space mapping techniques, deep domain adaptation can be divided into three major categories: Discrepancy-based, adversarial discriminative and adversarial generative models \cite{csurka2017domain}. In \emph{adversarial network-based domain adaptation} frameworks, an adversarial network is used to minimize the discrepancy between the feature embedding space of the source and the target domain by encouraging domain confusion with an adversarial objective \cite{csurka2017domain}. \cite{Tzeng_2015_ICCV} proposed a domain confusion based network that optimizes domain invariant with an adversarial network to facilitate domain adaptation from source to target domain using soft label distribution matching loss. The Domain-Adversarial Neural Network (DANN) \cite{ganin2016domain} introduces a gradient reversal layer which works adversarially to promote the emergence of features that are indiscriminate to domain shift from source domain to target domain. Some other frameworks use generative network along with the adversarial one in order to generate the mapping of common feature space. For example, in the Adversarial Discriminative Domain Adaptation (ADDA) \cite{tzeng2017adversarial}, an inverted label Generative Adversarial Network (GAN) loss is used to split the optimization into generative and discriminative objective. In cycle-consistent conditional adversarial transfer networks (3CATN) \cite{li2019cycle}, the conditioning of adversarial network with the cross-covariance of learned features and class labels are used to capture the multi-modal structure of data distribution and later for domain adaptation. A method of learning the domain invariant representation dynamically in terms of the relative importance of global and local feature importance is presented in \cite{yu2019transfer}. \emph{Discrepancy-based methods of domain adaptation} uses a discrepancy metric between the corresponding activation layers of two stream networks for source and target domains. In deep CORAL \cite{sun2016deep}, second order statistics of the source and the target distributions are aligned with linear transformation. Central Moment Discrepancy (CMD) is used as discrepancy metrics in \cite{zellinger2017central} to match the higher order central moment of probability distribution of the feature spaces. MMD based methods have been used to train the CNN to simultaneously minimize both the divergence and category loss for the source domain as well \cite{long2015learning,long16}.


%Although the adversarial and generative adversarial networks based domain adaptation frameworks achieve very good results in different domains of application, the training process is complex and does not guaranteed to be converged in case of high-dimensional signals like Lidar or Radar \cite{yao2019heterogeneous}. On the other hand, discrepancy-based methods related error on the target domain is bounded by the divergence of its distributions and related noises which make it difficult to learn a domain invariant feature space between heterogeneous source and target domain like Lidar and Radar \cite{ben07}. Our proposed \emph{SAEDA} framework uses a modified MMD called Class-wise MMD metric to minimize distance between the bottleneck feature representation of source and target auto-encoder. To our understanding, these distribution aligning methods using adversarial network- or discrepancy- based methods do not consider of using auto-encoders for aligning domain invariant common feature space. There are several auto-encoder based methods proposed by researchers as well. Ghifary et al. proposed using an autoencoder for the target domain to obtain domain-invariant features \cite{Ghifary16}. Sener et al. proposed using clustering techniques and pseudo-labels to obtain discriminative features \cite{Sener16}. Considering matching distributions of the bottleneck features space of auto-encoders to be effective in realizing an accurate adaptation, we propose a simultaneous training mechanism of auto-encoders (source and target). To best of our knowledge, \emph{SAEDA} is the first of its kind that consider simultaneous learning scheme of source and target auto-encoders with careful design of modified MMD loss across the domain invariant feature space.


%\par As stated earlier, almost all of the discrepancy based domain adaptation frameworks align the feature space at some layers in the middle of a classification network.

% \begin{figure}[!htb]

% \begin{center}
%   \includegraphics[width=\linewidth]{feat_space.png}
%   \caption{Feature representations space of a. Classification stream network, b. Auto-encoder network.}
%   \label{feat_rep}
% \end{center}
% \end{figure}


%\par In figure \ref{feat_rep} we show intuitively how the feature representation space of our auto-encoder framework differs from the feature representation space of the classification stream network. In classification stream network, the samples of same class cluster together because it is an intermediate stage of an classification network. Because of clustering most of the samples in the feature representation space $\hat{X}$ of the same class lose one to one relationship with the input features $X$. As a result, the domain adaptation with the discrepancy based methods in this feature space only works with the centroids of the clusters of different classes rather than with the individual samples. This can result to negative transfer when there are heterogeneity present with the class labels.

%\par On the other hand, the representation space of the bottleneck layer of deep auto-encoder is not clustered. The feature representation space is scattered because of the nature of the of the optimization function. One to one relationship also hold between the input features $X$ and the feature representation space $\hat{X}$. As a result, during the domain adaptation optimization, transfer of features from the source to the target domain occurs all over the regions of feature representation space rather than just in the clusters of classes. This way domain adaptation with auto-encoder can achieve state-of-the-art performance using a simple training scheme.

% \begin{figure}
%   \centering
%   \includegraphics[width=\linewidth]{autoencoder_arch.png}
%   \caption{Network architecture of the source and the target auto-encoder.}
%   \label{network_arc}
% \end{figure}


%\begin{table*}[t]
%  \caption{Domain adaptation performance comparisons on our collected three datasets while $\rightarrow$ denotes the source to target domain adaptation.}
%  \label{result-table}
 % \centering
 % \begin{tabular}{llllll}
%    \toprule
%   \multicolumn{2}{c}{Part}                   \\
%    \cmidrule(r){1-2}
%    Method     & Radar$\rightarrow$Lidar  & Lidar$\rightarrow$Radar    & Radar+Lidar$\rightarrow$Radar & Radar+Lidar$\rightarrow$Lidar & Avg\\
%    \midrule
%    Source & $67.3\pm0.3$ & $62.8\pm0.2$ & $66.4\pm0.4$ & $89.7\pm0.2$ & 71.6\\
%    Target & $67.3\pm0.3$ & $62.8\pm0.2$ & $66.4\pm0.4$ & $89.7\pm0.2$ & 71.6\\
 %   HDCNN \cite{tzeng2014deep} & $71.9\pm0.4$  & $78.4\pm0.1$ & $75.8\pm0.3$ & $89.9\pm0.2$  & 79.0\\
 %   CORAL \cite{long2015learning} & $79.5\pm0.3$ & $79.6\pm0.2$ & $89.8\pm0.2$ & $75.2\pm0.1$ & 81.0\\
%    CGAN \cite{ganin2016domain} & $70.6\pm0.2$ & $76.7\pm0.4$ & $76.6\pm0.3$ & $90.2\pm0.2$ & 78.5\\
 %   \textbf{SAEDA(Ours)} & $\mathbf{95.22}\pm0.3$ & $\mathbf{85.7}\pm0.2$ & $93.8\pm0.2$ & $\mathbf{96.6}\pm0.2$ & $\mathbf{92.8}$\\
%    
 %   \bottomrule
%  \end{tabular}
%\end{table*}


%Our \emph{SAEDA} framework outperformed all other state-of-the-art methods in all of the domain adaptation scenarios except CORAL in USPS$\rightarrow$MNIST. It is worth to note that, in case of SVHN$\rightarrow$MNIST, \emph{SAEDA} outperformed all other algorithms with a significant margin where source and target images are mostly dissimilar. 
%\par The performance of the discrepancy based methods (DDC, DAN, CMD, CORAL) is significantly superior than the baseline Convolution neural network based Modified LeNet model which confirms the effectiveness of these models to reduce domain discrepancy. On the other hand, adversarial domain adaptation methods (DANN, ADDA) also outperformed the baseline method. However, their performance varies widely among different domain adaptation scenarios which shows their lack of robustness with the variation of domains. Finally, \emph{SAEDA} outperforms all of the baseline methods on nearly all of the domain adaptation scenarios as well as on the average performance. This confirms the ability of the \emph{SAEDA} framework to minimize the domain discrepancy efficiently with a simple and stable training procedure. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{figure*}
%     \centering
%     \begin{subfigure}[b]{0.57\textwidth}
%         \centering
%         \includegraphics[width=\textwidth]{learning_curve.png}
 %       \caption{}
 %        \label{fig:convergence}
 %    \end{subfigure}
 %    \hfill
 %    \begin{subfigure}[b]{0.42\textwidth}
 %        \centering
 %        \includegraphics[width=\textwidth]{target_frac_v_acc.png}
 %        \caption{}
 %        \label{fig:fraction_convergence}
 %    \end{subfigure}
%        \caption{(a) Comparison of SAEDA convergence performance with baseline algorithms LS-ADDA (Least Square ADDA), DI (Domain Invariance LS-ADDA) and DIFA(Domain Invariance and Feature Augmentation LS-ADDA), (b) Domain adaptation performance changes on different sample size (fraction of samples) of target data}
%        \label{fig:three graphs}
%\end{figure*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Performance Analysis}
%\subsection{Bottleneck Space visualization}
%To validate the theoretical assumption described in figure \ref{feat_rep}, we visualize the bottleneck representation space of the auto-encoders of our proposed framework in theorems 1-3. After the completion of training the auto-encoders, we randomly took 2000 samples from MNIST and USPS data-set and get 100 dimensional representation space from the bottleneck layer. We use principal component analysis to extract two principal components from that 100 dimensional space. For easy and simple visualization, we present 3 classes in a single graph.
%\par In figure \ref{rep_s}, we observe a smooth transition between different classes rather than clustered centroids. Yet there is a clear distinction between different classes. As we mentioned earlier, this helps to obtain domain adaptation along a wide region of bottleneck representation space. As a result, adaptation through domains having very distinct features can be possible with higher accuracy.

%\subsection{Convergence Performance}
%To compare the stability of our system, we compared the convergence performance of \emph{SAEDA} with three variations of ADDA \cite{tzeng2017adversarial} described in \cite{Volpi_2018_CVPR}: LS-ADDA (Least Square ADDA), DI (Domain Invariance LS-ADDA) and DIFA(Domain Invariance and Feature Augmentation LS-ADDA), as shown in Fig. \ref{fig:convergence}. In case of both SVHN$\rightarrow$MNIST and USPS$\rightarrow$MNIST, our \emph{SAEDA} model showed higher stability and higher score. In case of SVHN$\rightarrow$MNIST, our model converged way faster than all three other variations of ADDA. This validates the theoretical assumption of higher stability of our model compared to adversarial network-based methods. Fig. \ref{fig:fraction_convergence} shows the convergence of \emph{SAEDA} variants of the target labels (fraction) which provides ample proof that \emph{SAEDA} adapts fast enough to be considered as a simple solution against the complexity of training and uncertainty of domain invariant feature spaces of other methods.
